Boosting Diffusion Models with an Adaptive Momentum Sampler

Diffusion probabilistic models (DPMs) have been shown to generate high-quality images without the need for delicate adversarial training. However, the current sampling process in DPMs is prone to violent shaking. In this paper, we present a novel reverse sampler for DPMs inspired by the widely-used Adam optimizer. Our proposed sampler can be readily applied to a pre-trained diffusion model, utilizing momentum mechanisms and adaptive updating to smooth the reverse sampling process and ensure stable generation, resulting in outputs of enhanced quality. By implicitly reusing update directions from early steps, our proposed sampler achieves a better balance between high-level semantics and low-level details. Additionally, this sampler is flexible and can be easily integrated into pre-trained DPMs regardless of the sampler used during training. Our experimental results on multiple benchmarks demonstrate that our proposed reverse sampler yields remarkable improvements over different baselines. We will make the source code available.

==> tab/ablation.tex <==
\begin{table}[!htpb]
    %\vskip -0.1in
    \caption{CelebA image generation results measured in FID $\downarrow$ with basic momentum and adaptive momentum. The best results of each column are shown in bold.}
    \centering
    %\vspace{0.2cm}
    \resizebox{\linewidth}{!}{
        \begin{tabular}{l|cccc}
            \toprule
            & \multicolumn{4}{c}{CelebA} \\
            dim($\tau$) & 25 & 50 & 100 & 1000 \\
            \midrule
            DDPM ($\eta = 1$) & 24.32 & 17.86 & 13.54 & 5.78\\
            DDPM + M & 23.20 & \textbf{16.41} & 11.62 & 3.41  \\
            DDPM + AM & \textbf{23.10} & 16.42 & \textbf{10.94} & \textbf{2.50} \\
            \bottomrule
        \end{tabular}
}
%\vskip 0.1in
\label{tab:ablation}
\end{table}

==> tab/celeba.tex <==
\begin{table}[!htpb]
    %\vskip -0.1in
    \caption{CelebA image generation results, measured in FID $\downarrow$.}
    \centering
    %\vspace{0.2cm}
    \resizebox{\linewidth}{!}{
        \begin{tabular}{l|ccccc}
            \toprule
            & \multicolumn{5}{c}{CelebA} \\
            dim($\tau$) & 1000 & 100 & 50 & 25 & 10 \\
            \midrule
            DDIM ($\eta = 0$) & \framebox[1.1\width]{3.40} & \framebox[1.1\width]{6.25} & \framebox[1.1\width]{9.08} & \framebox[1.1\width]{11.88} &  \\
            DDIM + M & 3.26 & 6.21 & 8.65 & 12.01  &  \\
            DDIM + Adam & 3.59 & 6.59 & 9.15 &  &  \\
            \midrule
            DDPM ($\eta = 1$) & 5.78 & 13.54 & 17.86 &  &  \\
            DDPM + M & 3.41 & 11.62 & \framebox[1.1\width]{16.41} &  &  \\
            DDPM + Adam & \framebox[1.1\width]{2.50} & \framebox[1.1\width]{10.94} & 16.42  &  &  \\
            \midrule
            DDPM ($\eta = \hat{\eta}$) & 3.37 & 46.66 & 72.96 & 145.71 &  \\
            DDPM + M  & 3.36 & \framebox[1.1\width]{46.52} & 69.93 & 145.74 &  \\
            DDPM + Adam & \framebox[1.1\width]{3.17} & 46.68 & \framebox[1.1\width]{68.40} &  &  \\
            \bottomrule
        \end{tabular}
}
%\vskip 0.1in
\label{tab:celeba}
\end{table}

==> tab/hyperparameters-all.tex <==
\begin{table}[!htpb]
    %\vskip -0.1in
    \caption{Hyperparameter setting for CIFAR10, ImageNet, Celeb-A, LSUN Church and Bedroom with different methods}
    \centering
    %\vspace{0.2cm}
    \resizebox{\linewidth}{!}{
        \begin{tabular}{l|l|cccccc}
            \toprule[2pt]
            Method & & CIFAR10 & ImageNet & Celeb-A & Church & Bedroom \\
            \midrule[2pt]
            \multirow{2}{*}{
            \begin{tabular}[c]{@{}l@{}}
            DDIM + AM \\ ($\eta = 0$)
            \end{tabular}} & $b_{\max}$ & 0.4 & $1 \times 10^{-3}$ & $1 \times 10^{-3}$ & $3 \times 10^{-3}$  & $1.5 \times 10^{-3}$ \\
            \cline{2-7}
            & $c$ & 0.9999 & 0.9999 & 0.9999 & 0.9999 & 0.9999 \\
            \midrule[2pt]
            \multirow{2}{*}{
            \begin{tabular}[c]{@{}l@{}}
            DDPM + AM \\ ($\eta = 1$)
            \end{tabular}} & $b_{\max}$ & 0.15 & $1 \times 10^{-3}$ & 0.15 & 0.01 & 0.05 \\
            \cline{2-7}
            & $c$ & 0.99 & 0.9999 & 0.9 & 0.999 & 0.999 \\
            \midrule[2pt]
            \multirow{2}{*}{
            \begin{tabular}[c]{@{}l@{}}
            DDPM + AM \\ ($\eta = \hat{\eta}$)
            \end{tabular}} & $b_{\max}$ & 0.125 & $1 \times 10^{-3}$ & $1 \times 10^{-3}$ & - & - \\
            \cline{2-7}
            & $c$ & 0.9999 & 0.9999 & 0.9 & - & - \\
            \bottomrule[2pt]
        \end{tabular}
}
%\vskip 0.1in
\label{tab:hyper-all}
\end{table}

==> tab/main_fid.tex <==
\begin{table*}[!htpb]
    %\vskip -0.1in
    \caption{The image generation results on CIFAR10 (32 $\times$ 32), ImageNet (64 $\times$ 64), Celeb-A (64 $\times$ 64), Church (256 $\times$ 256) and Bedroom (256 $\times$ 256), measured in IS $\uparrow$ and FID $\downarrow$.
    Note that a same pre-trained diffusion model is utilized on each dataset with different sampling strategies. 
    The improvement of the adaptive momentum sampling (`+AM') is remarkable on most of the datasets compared to the baselines in terms of FID.
    It is reasonable for our method to have similar IS to baselines, since the adaptive momentum mainly smooth the sampling trajectory which have no impact on changing the labels of the image, while IS is sensitive to inter-class diversity only.
    }
    \centering
    %\vspace{0.2cm}
    \resizebox{0.85\linewidth}{!}{
        \begin{tabular}{l|cccccccc}
            \toprule[2pt]
            & \multicolumn{2}{c}{CIFAR10} & \multicolumn{2}{c}{ImageNet} & Celeb-A & Church & Bedroom \\
            Sampler & IS & FID & IS & FID & FID & FID & FID \\
            \midrule[2pt]
            DDIM ($\eta = 0$) & 8.16 $\pm$ 0.15 & 3.98 & 16.40 $\pm$ 0.25 & 19.09 & 3.40 & 10.84 & 7.39 \\
            Analytic-DDPM  & - & 4.66 & - & 18.98 & \textbf{3.13} & - & -  \ML[0.08em] 
            DDIM + AM & 8.16 $\pm$ 0.15 & \textbf{3.81} & 16.35 $\pm$ 0.28 & \textbf{18.85} & 3.24 & \textbf{8.17} & \textbf{5.91}  \\
            \midrule[2pt]
            DDPM ($\eta = 1$) & 8.22 $\pm$ 0.09 & 4.72 & 17.14 $\pm$ 0.20 & 16.55 & 5.78 & - & - \\
            Analytic-DDPM & - & 4.31 & - & \textbf{16.34} & 5.21 & - & - \ML[0.08em]
            DDPM + AM & 8.41 $\pm$ 0.09 & \textbf{3.53} & 17.14 $\pm$ 0.21 & 16.51 & \textbf{2.50} & - & - \\
            \midrule[2pt]
            DDPM ($\eta = \hat{\eta}$) & 8.39 $\pm$ 0.15 & 3.16 & 17.15 $\pm$ 0.18 & 16.38 & 3.26 & 7.81 & 6.24 \\
            Analytic-DDPM & - & 4.31 & - & 16.34 & 5.21 & - & - \ML[0.08em]
            DDPM + AM  & 8.46 $\pm$ 0.08 & \textbf{3.14} & 17.15 $\pm$ 0.19 & \textbf{16.29} & \textbf{3.17} & \textbf{7.74} & \textbf{5.54} \\
            \bottomrule[2pt]
        \end{tabular}
}
%\vskip 0.1in
\label{tab:main_exp}
\end{table*}
